Generalized Fast Multichannel Nonnegative Matrix Factorization Based on Gaussian Scale Mixtures for Blind Source Separation

This paper describes heavy-tailed extensions of a state-of-the-art versatile blind source separation method called fast multichannel nonnegative matrix factorization (FastMNMF) from a unified point of view. The common way of deriving such an extension is to replace the multivariate complex Gaussian distribution in the likelihood function with its heavy-tailed generalization, e.g., the multivariate complex Student's t and leptokurtic generalized Gaussian distributions, and tailor-make the corresponding parameter optimization algorithm. Using a wider class of heavy-tailed distributions called a Gaussian scale mixture (GSM), i.e., a mixture of Gaussian distributions whose variances are perturbed by positive random scalars called impulse variables, we propose GSM-FastMNMF and develop an expectationmaximization algorithm that works even when the probability density function of the impulse variables have no analytical expressions. We show that existing heavy-tailed FastMNMF extensions are instances of GSM-FastMNMF and derive a new instance based on the generalized hyperbolic distribution that include the normal-inverse Gaussian, Student's t, and Gaussian distributions as the special cases. Our experiments show that the normalinverse Gaussian FastMNMF outperforms the state-of-the-art FastMNMF extensions and ILRMA model in speech enhancement and separation in terms of the signal-to-distortion ratio.

==> geo_SDR_RT60.tex <==
\begin{table*}
\setlength{\tabcolsep}{5.7pt}
\setlength{\aboverulesep}{1pt}
\setlength{\belowrulesep}{1pt}
\begin{centering}
\caption{
The SDRs (mean $\pm$ standard deviation) 
obtained by the eight methods in speech enhancement for $M=8$ and various $RT_{60}$.
}\label{tab:geo_enhancement_sdr_RT60}
\vspace{-2mm}
\begin{tabular}{@{}lcc*{8}{r}@{}}
\toprule
\multirow{2}{*}[-2pt]{Dist.} & \multirow{2}{*}[-2pt]{SNR} & \multirow{2}{*}[-2pt]{$RT_{60}$ [s]} & \multicolumn{4}{c}{{FastMNMF variants}} & \multicolumn{4}{c}{{R1-FastMNMF variants}} \\
\cmidrule(lr){4-7} \cmidrule(lr){8-11}
  &  &  &
  \multicolumn{1}{c}{$\mathcal{N}$} & 
  \multicolumn{1}{c}{$t$} &
  \multicolumn{1}{c}{GG} & 
  \multicolumn{1}{c}{NIG} &
  \multicolumn{1}{c}{$\mathcal{N}$} & 
  \multicolumn{1}{c}{$t$} &
  \multicolumn{1}{c}{GG} & 
  \multicolumn{1}{c}{NIG}  \\
\midrule
% old order: NIG GG t N R1-NIG R1-GG R1-t R1-N
% new-order : N t GG NIG R1-N R1-t R1-GG R1-NIG
\multirow{9}{*}[-2pt]{Near} & \multirow{3}{*}{$0$~dB} & 0.25 &
$14.3~(\pm 4.2)$ &
$13.8~(\pm 3.2)$ &
$15.9~(\pm 4.6)$ &
$\mathbf{16.5~(\pm 4.3)}$ &
$11.9~(\pm 2.9)$ &
$12.2~(\pm 3.3)$ & 
$11.6~(\pm 2.6)$ & 
$12.6~(\pm 2.8)$
 \\
 &  & 0.50 &
$11.1~(\pm 4.1)$ &
$11.0~(\pm 3.8)$ &
$12.0~(\pm 4.4)$ &
$\mathbf{12.9~(\pm 4.2)}$ & 
$7.1~(\pm 2.1)$ & 
$7.9~(\pm 2.7)$ & 
$7.6~(\pm 3.2)$ & 
$8.3~(\pm 2.3)$
 \\
 
 &  &  0.70 &
$10.7~(\pm 3.8)$ &
$7.7~(\pm 2.9)$ &
$10.4~(\pm 3.9)$ & 
$\mathbf{11.1~(\pm 4.5)}$ & 
$5.6~(\pm 2.4)$ &  
$7.1~(\pm 3.2)$ &  
$6.6~(\pm 3.9)$ &  
$7.7~(\pm 3.0)$
 \\
 
 \cmidrule(lr){2-11}
 & \multirow{3}{*}{$5$~dB} & 0.25 &
$18.0~(\pm 3.2)$ & 
$16.7~(\pm 2.6)$ & 
$18.1~(\pm 3.3)$ &  
$\mathbf{18.4~(\pm 3.3)}$ & 
$14.9~(\pm 2.5)$ &  
$15.2~(\pm 2.7)$ &  
$14.2~(\pm 3.6)$ & 
$15.4~(\pm 2.8)$
 \\
 &  &  0.50 &  
$13.1~(\pm 3.0)$ &
$13.3~(\pm 2.4)$ &
$14.8~(\pm 3.1)$ &
$\mathbf{15.8~(\pm 4.2)}$ &
$11.2~(\pm 2.5)$ & 
$11.2~(\pm 3.0)$ & 
$11.7~(\pm 2.9)$ &
$13.0~(\pm 2.3)$ 
 \\
 &  &  0.70 & 
$12.3~(\pm 3.4)$ & 
$12.2~(\pm 3.0)$ &
$\mathbf{14.2~(\pm 3.2)}$ &
$13.8~(\pm 3.2)$ & 
$9.1~(\pm 2.0)$ & 
$11.0~(\pm 2.8)$ & 
$10.7~(\pm 1.9)$ & 
$11.6~(\pm 2.6)$
\\
 
 \cmidrule(lr){2-11}
 & \multirow{3}{*}{$10$~dB} & 0.25 &
$19.5~(\pm 3.8)$ &
$18.7~(\pm 2.3)$ & 
$19.1~(\pm 3.3)$ &
$\mathbf{19.9~(\pm 2.8)}$ &
$18.0~(\pm 2.1)$ &  
$17.2~(\pm 3.1)$ &  
$16.2~(\pm 2.7)$ &  
$18.5~(\pm 3.1)$
 \\
 &  &  0.50 &  
$13.9~(\pm 2.7)$ &
$14.3~(\pm 2.3)$ &
$16.8~(\pm 2.8)$ &
$\mathbf{17.1~(\pm 3.1)}$ &  
$14.2~(\pm 2.5)$ & 
$12.1~(\pm 6.9)$ &
$13.5~(\pm 2.7)$ & 
$13.8~(\pm 4.6)$\\
 
 &  &  0.70 &
$12.3~(\pm 1.9)$ & 
$14.2~(\pm 2.4)$ &
$15.0~(\pm 2.5)$ & 
$\mathbf{15.8~(\pm 3.4)}$ & 
$11.6~(\pm 2.1)$ &
$11.2~(\pm 2.6)$ & 
$10.6~(\pm 5.7)$ &  
$13.6~(\pm 2.3)$
 \\
 \midrule 
\multirow{9}{*}[-2pt]{Far} & \multirow{3}{*}{$0$~dB} & 0.25 &
$9.9~(\pm 3.4)$ & 
$7.8~(\pm 3.5)$ & 
$10.2~(\pm 4.4)$ & 
$\mathbf{10.9~(\pm 3.8)}$ &  
$8.3~(\pm 3.4)$ &  
$8.0~(\pm 3.4)$ & 
$7.0~(\pm 3.1)$ &  
$9.0~(\pm 2.4)$
\\
 &  & 0.50 &
$4.9~(\pm 3.9)$ & 
$5.9~(\pm 3.6)$ & 
$6.8~(\pm 3.6)$ &
$\mathbf{7.0~(\pm 4.1)}$ & 
$3.9~(\pm 2.1)$ & 
$3.7~(\pm 2.7)$ & 
$4.5~(\pm 3.3)$ &
$5.0~(\pm 2.9)$
\\
 &  & 0.70 &
$4.0~(\pm 4.7)$ &
$4.6~(\pm 3.0)$ &
$6.2~(\pm 4.3)$ & 
$\mathbf{6.6~(\pm 3.8)}$ &  
$0.9~(\pm 2.4)$ &  
$3.5~(\pm 2.7)$ &  
$3.2~(\pm 3.6)$ &  
$4.2~(\pm 3.0)$
\\
\cmidrule(lr){2-11}
& \multirow{3}{*}{$5$~dB} & 0.25 &
 $11.7~(\pm 4.1)$ & 
 $11.3~(\pm 3.3)$ & 
 $11.7~(\pm 3.5)$ & 
 $\mathbf{12.2~(\pm 3.9)}$ & 
 $10.0~(\pm 2.8)$ & 
 $10.2~(\pm 2.8)$ & 
 $9.7~(\pm 4.9)$ &  
 $9.5~(\pm 3.0)$
\\
&  & 0.50 &
$6.8~(\pm 3.1)$ & 
$7.0~(\pm 2.7)$ & 
$\mathbf{8.7~(\pm 3.5)}$ & 
$8.5~(\pm 3.5)$ & 
$5.8~(\pm 3.5)$ &
$6.4~(\pm 3.2)$ & 
$6.3~(\pm 2.4)$ &  
$8.0~(\pm 4.1)$
 \\
 &  & 0.70 &
$5.8~(\pm 3.3)$ & 
$7.0~(\pm 3.6)$ & 
$8.2~(\pm 3.8)$ &
$\mathbf{8.3~(\pm 3.4)}$ &  
$3.9~(\pm 3.9)$ &  
$4.6~(\pm 3.2)$ & 
$5.5~(\pm 3.2)$ & 
$7.3~(\pm 2.6)$ 
\\

\cmidrule(lr){2-11}
& \multirow{3}{*}{$10$~dB} & 0.25 &
$13.0~(\pm 3.0)$ &
$12.0~(\pm 3.2)$ & 
$\mathbf{13.8~(\pm 3.8)}$ &
$13.7~(\pm 3.8)$ &  
$12.1~(\pm 4.1)$ & 
$11.8~(\pm 3.1)$ & 
$9.6~(\pm 3.7)$ & 
$11.2~(\pm 3.9)$
\\
&  &  0.50 & 
$8.7~(\pm 3.8)$ &
$\mathbf{10.1~(\pm 2.8)}$ &  
$9.4~(\pm 2.9)$ &
$9.8~(\pm 4.0)$ &
$9.1~(\pm 3.0)$ &  
$6.8~(\pm 2.3)$ & 
$7.5~(\pm 3.2)$ &
$8.5~(\pm 3.3)$
\\
&  &  0.70 &
$5.0~(\pm 3.6)$ &
$7.6~(\pm 3.6)$ &
$\mathbf{9.0~(\pm 3.8)}$ & 
$8.3~(\pm 2.7)$ & 
$4.9~(\pm 4.1)$ & 
$4.7~(\pm 4.9)$ & 
$7.3~(\pm 4.0)$ & 
$7.9~(\pm 2.6)$
\\
\bottomrule
\end{tabular}
\par\end{centering}
\end{table*}





